A Unified Framework for Pun Generation with Humor Principles

We propose a unified framework to generate both homophonic and homographic puns to resolve the split-up in existing works. Specifically, we incorporate three linguistic attributes of puns to the language models: ambiguity, distinctiveness, and surprise. Our framework consists of three parts: 1) a context words/phrases selector to promote the aforementioned attributes, 2) a generation model trained on non-pun sentences to incorporate the context words/phrases into the generation output, and 3) a label predictor that learns the structure of puns which is used to steer the generation model at inference time. Evaluation results on both pun types demonstrate the efficacy of our model over strong baselines.

==> 01-old-intro.tex <==
%Computational theories for puns have emerged in recent years. \citet{kao2016computational} use a probabilistic model to decompose puns into two dimensions: \textbf{ambiguity} of meaning and \textbf{distinctiveness} of viewpoints, and show that these two aspects combined have statistically significant alignment with humans judgments. For example, in Figure \ref{fig:illustration}, `cab' is distinct to the pun word `taxi', whereas `tell' is ambiguous because it supports both `taxi' and the alternative word, `tax'. However, the NLG community has only witnessed sporadic attempts to include related words for semantic relevance of generated puns \cite{mittal2022ambipun,  yu2018neural,yu-etal-2020-homophonic}. The incorporation of ambiguity and distinctiveness principles to generation models is still lacking, because of the difficulty in measuring ambiguity/distinctiveness automatically.

%Likewise, \citet{he2019pun} %propose retrieve-and-edit pipelines to generate puns. \citet{he2019pun} mathematically formulate the intuition that the pun word (`taxi') should be unexpected in the local context (seeing `get into all that \textit{tax} trouble' is more expected) while making sense in the global context. Although the proposed local-global \textbf{surprisal} principle shows strong correlation with human preference, their error analysis shows that the proposed phrase retrieval methods are sometimes incompatible or too vague.

We hypothesize that there is a learnable structure for puns regardless of the pun type, and propose a unified pun generation framework that incorporates all three principles: ambiguity, distinctiveness, and surprise. Specifically, we carefully extract a 'context word that supports the pun word, and a phrase that is both characteristic to the alternative word and compatible with the pun word (e.g. `get in all that tax trouble') to arouse surprise. Next, we train a discriminator on existing homophonic pun data to learn the structure of a pun-- the \textit{type} of each word in the sentence, which could be one of `A'- ambiguous, `D1'- distinct to the pun word, or `D2'- distinct to the alternative word. The challenge is that there is no ground truth labels. To this end, we collect a small amount of human annotations and boost from weak, unsupervised models to stronger, supervised models (in Section \ref{subsec:label_curation}). At inference time, the same label predictor is used to guide the base language model (i.e., GPT-2) to generate puns. At each generation step, the label predicted is either D1, D2 or A. We re-score the tokens generated by the base language model based on the predicted label, and do not intervene the base language model if the label predictor is less confident. Our model outperforms existing baselines for both pun types.

Moreover, existing works are split up in terms of generating homographic puns, wherein the same written word has two or more meanings \cite{mittal2022ambipun, yu-etal-2020-homophonic, yu2018neural} and homophonic puns, where two words that sound similar have different meanings \cite{luo2019pun, he2019pun, hashimoto2018retrieveandedit}. In this work, we bridge the gap between these two pun types by converting homographic puns to homophonic ones.

